Rethinking Theory of Mind Benchmarks for LLMs: Towards A User-Centered Perspective

The last couple of years have witnessed emerging research that appropriates Theory-of-Mind (ToM) tasks designed for humans to benchmark LLM's ToM capabilities as an indication of LLM's social intelligence. However, this approach has a number of limitations. Drawing on existing psychology and AI literature, we summarize the theoretical, methodological, and evaluation limitations by pointing out that certain issues are inherently present in the original ToM tasks used to evaluate human's ToM, which continues to persist and exacerbated when appropriated to benchmark LLM's ToM. Taking a human-computer interaction (HCI) perspective, these limitations prompt us to rethink the definition and criteria of ToM in ToM benchmarks in a more dynamic, interactional approach that accounts for user preferences, needs, and experiences with LLMs in such evaluations. We conclude by outlining potential opportunities and challenges towards this direction.

==> deleted.tex <==
ToM dimensions evaluated in LLM: one-dimensional on false beliefs, multi-dimensional such as BDI dimensions~\cite{chan2024negotiationtom}

Kinds of ToM tasks or data set: 
~\cite{soubki2024views}: use existing multi-turn conversation dialogues, annotated with beliefs. Presented as scenarios to LLM
~\cite{chan2024negotiationtom} used human-human bilateral natural conversational dataset, multi-turn dialogue. Adopted strategy annotations and undertake BDI annotation behind each utterance. Annotated by five graduate students. Tested through (1) zero-shot prompting and formulate as multiple choice question answering problems (2) CoT prompting using the prompt let's think step by step. (3) also used few-shot to see whether LLM can improve performance with input-output exemplars. 
~\cite{kim2023fantom}: conversation-based TOM evaluation to align with real-world scenarios. Reiterative questions at various levels for the same input context including free-form response, multiple-choice questions, and straightforward yes or no questions. 32 annotators on MTurk to annotate the entire conversation in the dataset. 
~\cite{hou2024entering}: from first-person perspective. Dynamic multi-turn interactive scenarios. Systematically transformed third person benchmarks into first-person perspective. RUle-based agents to mimic human cognitive behaviors. Socially interactive situations. Established human performance baseline. 
~\cite{shi2024muma}: multi-modal ToM benchmark. Provide video and text descriptions of people's multi-modal behavior in realistic household environment, then ask questions about people's goals and beliefs. Embodied multi-agent interactions. Validated the benchmark in a human experiment to provide human baseline. 


~\cite{sap2022neural}: two benchmarks: one using socialiqa~\cite{sap2019socialiqa} that presents social situations and questions to LLM to measure social commonsense and emotional intelligence; and tomI reasoning about people's mental states and realities~\cite{le2019revisiting}
~\cite{he2023hi}: automatically generate higher-order ToM stories, multiple choice, QA format. Stories generated based on a fixed structure. 
~\cite{xu2024opentom}: generated stories of characters with varying motivated actions, QA format. Stories look similar to Sally-Anne task


~\cite{le2019revisiting}: over 1000 distinct stories and questions regarding memory, reality, and 1st and 2nd order false belief. Inspired by Sally-Anne test. 
~\cite{shapira2023well}: based on faux pas test. Stories created by experts and a small part created by chatgpt then rephrased and fixed by experts
~\cite{kosinski2023theory}: false-belief scenarios based on sally-anne test
~\cite{chen2024tombench}: ToM benchmark that covers 8 tasks and 31 ToM abilities. Multiple-choice question format. Build-from-scratch inventory, draw inspiration from daily social scenarios and manually create 2860 original test samples. Still largely inspired by existing human TOM tests. Tasks are skewed towards assessing belief and non-literal communication, instead of intention and abilities
